WKB Methods for Finite Difference Schrodinger Equations

In this thesis, we develop WKB techniques for the finite difference Schrodinger equation, following the construction of the WKB approach for the standard differential Schrodinger equation. In particular, we will develop an all-order WKB algorithm to get arbitrary hbar-corrections and construct a general quantum momentum, underlining the various properties of its coefficients and the quantities that will be used when constructing the quantization condition. In doing so, we discover the existence of additional periodic factors that need to be considered in order to obtain the most general solution to the problem at hand. We will then proceed to study the simplest non trivial example, the linear potential case and the Bessel functions, that provide a solution to the linear problem. After studying the resurgence properties of the Bessel functions from an analytical and numerical point of view, we will then proceed to use those results in order to build general connection formulae, allowing us to connect the local solutions defined on two sides of a turning point into a smooth solution on the whole real line. With those connection formulae, we will analyse a selection of problems, constructing the discrete spectrum of various finite difference Schrodinger problems and comparing our results with existing literature.

==> 1.cover_PT_draft.tex <==
\setcounter{page}{1} \pagenumbering{Alph}

% Add PDF bookmark 
\pdfbookmark[0]{Title}{Title}

%%% LOGO
\thispagestyle{empty}
\begin{flushleft} ~\\ \vspace{-12mm} \hspace{-12mm}  \includegraphics[width=50mm]{istlogo} 
 
 %%% Instituição
\centering
\LARGE \textbf{UNIVERSIDADE DE LISBOA \\ INSTITUTO SUPERIOR TÉCNICO}
%%% espaço sem gráficos
\vspace{30mm}

%%% Optional Image
%\vspace{10mm}
%~\\ \vspace{50mm} % gráficos
%\\ \begin{center} \includegraphics[height=50mm]{Cover/coverimage}  \end{center} % gráficos
 \vspace{5mm}
 
 %%% Titulo
\centering
\LARGE \textbf{Título da Tese que descreve o objeto de estudo.}
\\ \vspace{10mm}
\Large Subtítulo Opcional
\\ \vspace{15mm}
%\\ \vspace{25mm}  % NO SUBTITLE
\Large \textbf{Nome completo} \\
\vspace{4cm}

\begin{minipage}{\textwidth}
\begin{tabularx}{\textwidth}{ l @{ } l }
\large \textbf{Orientador} : & \textbf{Doutor} Nome completo\\
 \large \textbf{Co-Orientador} :  & \textbf{Doutor} Nome completo\\
 %&    ~~~~~~~~~~~~~~~~~~~~~~~~~~ large name\\
\end{tabularx}

\end{minipage}
%
\\ \vspace{27mm}
%\vspace{12mm}
\centering
\large \textbf{Tese especialmente elaborada para a obtenção do grau de Doutor em}\\
\large Engenharia Mecânica\\
%\\ \vspace{2mm}
\vspace{18mm}
\Large \textbf{Tese Provisória}
 
\vspace{15mm}

%\large \textbf{\todaythesis\today} \\
\large \textbf{November 2017} \\
\let\thepage\relax
\end{flushleft}
\pagebreak

